Policy Optimization for PDE Control with a Warm Start

Dimensionality reduction is crucial for controlling nonlinear partial differential equations (PDE) through a "reduce-then-design" strategy, which identifies a reduced-order model and then implements model-based control solutions. However, inaccuracies in the reduced-order modeling can substantially degrade controller performance, especially in PDEs with chaotic behavior. To address this issue, we augment the reduce-then-design procedure with a policy optimization (PO) step. The PO step fine-tunes the model-based controller to compensate for the modeling error from dimensionality reduction. This augmentation shifts the overall strategy into reduce-then-design-then-adapt, where the model-based controller serves as a warm start for PO. Specifically, we study the state-feedback tracking control of PDEs that aims to align the PDE state with a specific constant target subject to a linear-quadratic cost. Through extensive experiments, we show that a few iterations of PO can significantly improve the model-based controller performance. Our approach offers a cost-effective alternative to PDE control using end-to-end reinforcement learning.

==> theory.tex <==
%We study the sample complexity of Algorithm \ref{alg:DPfilter} by analyzing the number of samples required in solving each iteration. First, we summarize the optimization landscapes of each quadratic program in Algorithm \ref{alg:DPfilter}.    
%\begin{fact}\label{lemma:convex}
%	There exists constants $m, \psi > 0$ such that for all $h\in\{0, \cdots, N-1\}$, the objective function $\cJ_h(\bL_h)$ in \eqref{eqn:induction} is $m$-strongly convex and $\psi$-smooth in $\bL_h$.
%\end{fact}
%Fact \ref{lemma:convex} is a direct result of the quadratic objective function $\cJ_h(\bL_h)$. Then, we define the \texttt{PolicyOptimizer} in Algorithm \ref{alg:DPfilter} to be the vanilla PG update: 
%\begin{align}
%	 \bL_{h}' = \bL_{h} - \eta_h \cdot \nabla_{\bL_h}\cJ_h(\bL_{h}), \label{eqn:PG}
%\end{align}
%where $\eta_h > 0$ is a constant stepsize to be determined. The PG update \eqref{eqn:PG} can be implemented using zeroth-order techniques as described in Algorithm \ref{alg:estimator}. We provide the convergence analysis of \eqref{eqn:PG} in the exact case (i.e., when exact gradients are accessible) based on standard results in minimization over strongly-convex and smooth functions.
%
%\begin{fact}\label{lemma:convergence}
%	For all $h \in \{0, \cdots, N-1\}$ and a fixed $\epsilon > 0$, choose a constant stepsize $\eta \in (0,  1/\psi]$. Then, the deterministic PG update \eqref{eqn:PG} converges linearly to $\bL^*_h$ such that $\|\bL_{h, T_h} - \bL^*_h\|_F \leq \epsilon$ holds after a total number of $T_h\sim\cO(\log(\epsilon^{-1}))$ iterations.
%\end{fact}
%
%When the PG update \eqref{eqn:PG} is estimated by using a two-point zeroth-order oracle (cf., Algorithm \ref{alg:estimator}), its convergence rate is at most $\cO(\sqrt{n(m+n)})$ slower than that of the stochastic first-order PG update \cite{duchi2015optimal}, where $n(m+n)$ is the dimension of $\bL_h$ for all $h$. Furthermore, the stochastic PG update converges with a high probability at a $\cO(\epsilon^{-2})$ rate with respect to the error distance in strongly convex and smooth minimization problems (e.g., Proposition 1 of \cite{rakhlin2011making}). We present the sample complexity results in the following proposition.
%
%\begin{proposition}\label{prop:sample}
%	For all $h\in\{0, \cdots, N-1\}$, choose the smoothing radius $r_{h, i} \sim \cO(\sqrt{\epsilon}\cdot i^{-1})$ and the stepsize $\eta_{h, i}\sim \cO(i^{-1})$. Then, the zeroth-order PG update \eqref{eqn:PG} converges after $T_h \sim \tilde{\cO}(\epsilon^{-2}\cdot\log(\delta^{-1}))$ iterations in the sense that $\|\bL_{T_h} - \bL_h^*\|_F\leq \epsilon$ with a probability of at least $1-\delta$.
%\end{proposition}
%
%Combining Theorem \ref{theorem:KF_DP} with Proposition \ref{prop:sample}, we can conclude that if every one-step KF problem, for all $h \in \{0, \cdots, N-1\}$, is solved to the $\epsilon$-accuracy with a probability of $1-\delta$, then the FPG algorithm outputs a stabilizing $\tilde{\bL}_{N-1}$ that satisfies $\|\tilde{\bL}_{N-1} - \bL^*\|_F\sim\cO(\epsilon)$ with a probability of $1-N\delta$, where $\bL^*$ is an optimal time-invariant filter parameters to the infinite-horizon KF problem \eqref{eqn:inf_est}. 
